Evaluating the Knowledge Dependency of Questions

The automatic generation of Multiple Choice Questions (MCQ) has the potential to reduce the time educators spend on student assessment significantly. However, existing evaluation metrics for MCQ generation, such as BLEU, ROUGE, and METEOR, focus on the n-gram based similarity of the generated MCQ to the gold sample in the dataset and disregard their educational value. They fail to evaluate the MCQ's ability to assess the student's knowledge of the corresponding target fact. To tackle this issue, we propose a novel automatic evaluation metric, coined Knowledge Dependent Answerability (KDA), which measures the MCQ's answerability given knowledge of the target fact. Specifically, we first show how to measure KDA based on student responses from a human survey. Then, we propose two automatic evaluation metrics, KDA_disc and KDA_cont, that approximate KDA by leveraging pre-trained language models to imitate students' problem-solving behavior. Through our human studies, we show that KDA_disc and KDA_soft have strong correlations with both (1) KDA and (2) usability in an actual classroom setting, labeled by experts. Furthermore, when combined with n-gram based similarity metrics, KDA_disc and KDA_cont are shown to have a strong predictive power for various expert-labeled MCQ quality measures.

==> tables/removed_tables.tex <==
% % from: approach


% \begin{table}[ht]
% \begin{tabularx}{\columnwidth}{l|l}
% \toprule
% Notation               & Description                                                                           \\ 
% \midrule
% $Q_i$                  & Question $i$                                                      \\ 
% \\[-1em]
% $F_i$                  & Fact $i$                                                                   \\
% \\[-1em]
% $(Q_i, F_i)$                  & $Q_i$ given with $F_i$                                                                  \\
% \\[-1em]
% $KC_i$                  & KC required to solve $Q_i$                                                      \\ 
% \\[-1em]
% $R_{ij}^{q}$ & Response of Solver $j$ for $Q_i$                                                         \\
% \\[-1em]
% $R_{ij}^{f}$      & Whether Solver $j$ knows $F_i$                                            \\
% \\[-1em]
% $R_{ij}^{q+f}$                & Response of Solver $j$ for $(Q_i, F_i)$                                                 \\
% \bottomrule
% \end{tabularx}
% \normalsize
% \caption{ \label{tab:notations}
% Notations
% }
% \end{table}

% \begin{table*}[]
% \begin{tabular}{c|c|c|c}
% \hline
%             & OBQA                                                           & TabMCQ                                                                                          & SciQ                                                                                                                       \\ \hline
% Fact        & predators eat prey                                             & \begin{tabular}[c]{@{}c@{}}Urban sprawl creates \\ thermal pollution\end{tabular}               & \begin{tabular}[c]{@{}c@{}}Plant hormones are chemical signals \\ that control different processes in plants.\end{tabular} \\ \hline
% Question    & Predators eat                                                  & \begin{tabular}[c]{@{}c@{}}What type of pollution \\ does Urban sprawl create?\end{tabular}     & \begin{tabular}[c]{@{}c@{}}What chemical signals in plants \\ control different processes?\end{tabular}                    \\ \hline
% Answer      & bunnies                                                        & thermal pollution                                                                               & plant hormones                                                                                                             \\ \hline
% Distractors & \begin{tabular}[c]{@{}c@{}}lions\\ humans\\ grass\end{tabular} & \begin{tabular}[c]{@{}c@{}}air pollution\\ radioactive pollution\\ noise pollution\end{tabular} & \begin{tabular}[c]{@{}c@{}}produce hormones\\ nitrogen hormones\\ Human Hormones\end{tabular}                              \\ \hline
% \end{tabular}
% \caption{Sample Questions. For OBQA, additional fact "bunnies are prey" is required to solve the question. However, SciQ and TabMCQ are mainly composed of questions that can be solely answered from the given fact.}
% \end{table*}



% % from: experiments


% \begin{table*}[ht!]
% \begin{tabular}{c|cc}
% \toprule
% Dataset/Model & TabMCQ / DG                                                           & SciQ / KDDG                                                                                                                                                                                                        \\ \hline
% Fact          & A(n) Flies is a(n) omnivore.                                          & \begin{tabular}[c]{@{}c@{}}Assume a molecule must cross the plasma \\ membrane into a cell. The molecule is a \\ very large protein. How will it be transported\\ into the cell? Explain your answer.\end{tabular} \\ \hline
% Question      & Flies would be in the \_ category.                                    & \begin{tabular}[c]{@{}c@{}}Assume a molecule must cross \\ a plasma membrane into what?\end{tabular}                                                                                                               \\ \hline
% Answer        & omnivore                                                              & cell                                                                                                                                                                                                               \\ \hline
% Distractors   & \begin{tabular}[c]{@{}c@{}}vegan\\ carnivore\\ herbivore\end{tabular} & \begin{tabular}[c]{@{}c@{}}circle\\ atam\\ shell\end{tabular}                                                                                                                                                      \\ \hline
% Likert        & 3.0                                                                   & 1.71                                                                                                                                                                                                               \\ \hline
% KDA\_s        & 0.55                                                                  & 0.81                                                                                                                                                                                                               \\ \hline
% KDA\_h        & 0.69                                                                  & 0.93                                                                                                                                                                                                               \\ \hline
% BLEU          & 66                                                                    & 0.00   \\                                                                                                                                                                                                        
% \bottomrule
% \end{tabular}
% \caption{Bad examples}
% \label{tab: dg-badexample}
% \end{table*}

% \begin{table*}[]
% \begin{tabular}{c|cc}
%             & Human                                                            & T5-DG                                                          \\ \hline
% Fact        & \multicolumn{2}{c}{Coyoteite can be found in rocks}                                                                               \\ \hline
% Question    & \multicolumn{2}{c}{Where can Coyoteite be found?}                                                                                 \\ \hline
% Answer      & \multicolumn{2}{c}{rocks}                                                                                                         \\ \hline
% Distractors & \begin{tabular}[c]{@{}c@{}}scissors\\ spoons\\ pens\end{tabular} & \begin{tabular}[c]{@{}c@{}}plastic\\ wood\\ glass\end{tabular} \\ \hline
% Likert      & 3.29                                                             & 3.71                                                           \\ \hline
% KDA\_s      & 0.90                                                             & 0.90                                                           \\ \hline
% KDA\_h      & 1.00                                                             & 1.00                                                           \\ \hline
% BLEU        & 0.00                                                             & 0.00                                                          
% \end{tabular}
% \end{table*}
 
% \begin{table*}[]
% \begin{tabular}{@{}lllll@{}}
% \toprule
%       & Human               & KDDG               & DG                  & qg+dg               \\ \midrule
% obqa   & 100.0 / 0.39 / 2.71 & 5.98 / 0.36 / 2.36 & 15.41 / 0.39 / 2.27 & 10.19 / 0.41 / 1.93 \\
% tabMCQ & 100.0 / 0.77 / 2.77 & 24.11 / 0.73 / 2.5 & 38.63 / 0.76 / 2.84 & 36.61 / 0.71 / 2.8  \\
% sciQ   & 100.0 / 0.9 / 2.79  & 9.9 / 0.88 / 2.84  & 18.06 / 0.84 / 2.88 & 18.4 / 0.86 / 2.79  \\ \bottomrule
% \end{tabular}
% \caption{ bleu / KDA / human likert score.}
% \end{table*}



% \begin{table*}[ht!]
% \begin{tabular}{@{}lllll@{}}
% \toprule
%                  & Irrelevant & Readability & Multiple Answer & Wrong Answer \\ \midrule
% not labeled only & 0.67**(51) & 0.64**(27)  & 0.19(44)        & 0.42**(72)   \\
% labeled only     & 0.06(45)   & 0.38**(69)  & 0.63**(52)      & 0.16(24)     \\ \midrule
% KDA-label corr   & -0.38**    & 0.17        & -0.22*          & -0.29**     
% \end{tabular}
% \caption{correlation between KDA and human likert score analyzed in specific groups. 'not labeled only' filters out the questions which is annotated to be rejected by certain reason. 'labeled only' groups contains rejected questions. number in () means number of samples. Last row shows the correlation between kda and the number of label. }
% \end{table*}




% \begin{table*}[]
% \begin{tabular}{@{}lll@{}}
% \toprule
% Label           & Question                                        & Type  \\ \midrule
% Answerability   & Is the question able to answer?                 & boolean   \\
% Multiple-answer & Does the question contain more than two answer? & boolean   \\
% Relavance       & Is the fact related to the question-solving?    & boolean   \\
% Personal usage  & Did you use the fact to the question-solving?   & boolean   \\
% hacking         & Can you infer the answer without using the fact?& boolean   \\
% ...             & ...                                             &        \\
% Quality         & How good is the question?                       & Likert \\
% Difficulty      & How difficult is the question?                  & Likert \\ \bottomrule
% \end{tabular}
% \caption{Questionnaire and type of each label. Boolean collects 0 or 1 value for each question, and likert-5 measures score between 1~5.}
% \label{table:label}
% \end{table*}





% \begin{table}[]
% \begin{tabular}{@{}lcc@{}}
% \toprule
% Label           & ACC         & F1 Score \\ \midrule
% Answerability   & 0.8         & 0.8      \\
% Multiple-answer & 0.9         & 0.8      \\
% Relavance       & 0.8         & 0.7      \\
% ...             & ...         & ...      \\ \midrule
% Label           & Correlation & AUC      \\ \midrule
% Quality         & 0.7         & 0.87     \\
% Difficulty      & 0.8         & 0.78     \\ \bottomrule
% \end{tabular}
% \caption{Label prediction performance. Accuracy and f1 score is applied to the boolean labels, while corrleation and AUC is applied to the likert scale labels.}
% \end{table}



% \begin{table*}[ht!]
% \begin{tabular}{@{}ccc|cc@{}}
% \hline
% \toprule
%                                   & \multicolumn{2}{c|}{Good}                                                                                                                              & \multicolumn{2}{c}{Bad}                                                                                                                                                                                                      \\ \midrule
% \multicolumn{1}{c|}{Dataset/Model} & \multicolumn{1}{c|}{TabMCQ / Human}                                                   & TabMCQ / T5-DG                                                 & \multicolumn{1}{c|}{TabMCQ / DG}                                                                   & SciQ / KDDG                                                                                                             \\ \midrule
% \multicolumn{1}{c|}{Fact}          & \multicolumn{2}{c|}{Coyoteite can be found in rocks}                                                                                                   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}A(n) Flies is \\ a(n) omnivore.\end{tabular}}       & \begin{tabular}[c]{@{}c@{}}Assume a molecule must \\ cross the plasma membrane \\ into a cell.. (continue)\end{tabular} \\ \midrule
% \multicolumn{1}{c|}{Question}      & \multicolumn{2}{c|}{Where can Coyoteite be found?}                                                                                                     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Flies would be \\ in the \_ category.\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Assume a molecule must \\ cross a plasma membrane \\ into what?\end{tabular}                 \\ \midrule
% \multicolumn{1}{c|}{Answer}        & \multicolumn{2}{c|}{rocks}                                                                                                                             & \multicolumn{1}{c|}{omnivore}                                                                      & cell                                                                                                                    \\ \midrule
% \multicolumn{1}{c|}{Distractors}   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}scissors\\ spoons\\ pens\end{tabular}} & \begin{tabular}[c]{@{}c@{}}plastic\\ wood\\ glass\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}vegan\\ carnivore\\ herbivore\end{tabular}}         & \begin{tabular}[c]{@{}c@{}}circle\\ atam\\ shell\end{tabular}                                                           \\ \midrule
% \multicolumn{1}{c|}{Likert}        & \multicolumn{1}{c|}{3.29}                                                             & 3.71                                                           & \multicolumn{1}{c|}{3.0}                                                                           & 1.71                                                                                                                    \\ \midrule
% \multicolumn{1}{c|}{KDA\_s}        & \multicolumn{1}{c|}{0.9}                                                              & 0.9                                                            & \multicolumn{1}{c|}{0.55}                                                                          & 0.81                                                                                                                    \\ \midrule
% \multicolumn{1}{c|}{KDA\_h}        & \multicolumn{1}{c|}{1.0}                                                              & 1.0                                                            & \multicolumn{1}{c|}{0.69}                                                                          & 0.93                                                                                                                    \\
% \multicolumn{1}{c|}{BLEU}          & \multicolumn{1}{c|}{100}                                                              & 0                                                              & \multicolumn{1}{c|}{66}                                                                            & 0.00                                                                                                                    \\ \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table}[]
% \begin{tabular}{c|cc|cc}
% \toprule
% Tree Depth      & \multicolumn{2}{c|}{2} & \multicolumn{2}{c}{3} \\ \hline
% Metrics    & +KDA         & -KDA       & +KDA        & -KDA       \\ \hline
% Accept    & \textbf{0.37}       & 0.02      & \textbf{0.41}      & 0.00      \\ \hline
% Likert    & \textbf{0.45}       & 0.09      & \textbf{0.44}      & 0.05      \\ \hline
% Irrelevant      & \textbf{0.29}       & -0.15     & \textbf{0.26}      & -0.09     \\ \hline
% Multi-ans. & 0.11       & \textbf{0.2}       & 0.13      & \textbf{0.17}      \\ \hline
% Readability     & -0.17      & \textbf{-0.01}     & -0.25     & \textbf{-0.01}     \\ \hline
% Wrong ans.    & \textbf{0.05}       & -0.24     & \textbf{0.09}      & -0.1      \\
% \bottomrule
% \end{tabular}
% \caption{Test set Pearson Correlation from Decision Tree. -KDA uses syntactic metrics only, and +KDA uses $KDA_S$ and $KDA_H$ as well.}
% \label{tab: examples}
% \end{table}


% \begin{table}[]
% \begin{tabular}{c|cc}
% \toprule
%             & \multicolumn{1}{c|}{H}                                                            & DG                                                          \\ \hline
% Fact        & \multicolumn{2}{c}{Coyoteite can be found in rocks}                                                                                                    \\ \hline
% Question    & \multicolumn{2}{c}{Where can Coyoteite be found?}                                                                                                      \\ \hline
% Answer      & \multicolumn{2}{c}{rocks}                                                                                                                              \\ \hline
% Distractors & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}scissors\\ spoons\\ pens\end{tabular}} & \begin{tabular}[c]{@{}c@{}}plastic\\ wood\\ glass\end{tabular} \\ \hline
% Likert      & \multicolumn{1}{c|}{3.29}                                                             & 3.71                                                           \\ \hline
% KDA\_s      & \multicolumn{1}{c|}{0.90}                                                             & 0.90                                                           \\ \hline
% KDA\_h      & \multicolumn{1}{c|}{1.00}                                                             & 1.00                                                           \\ \hline
% BLEU        & \multicolumn{1}{c|}{0.00}                                                             & 0.00                                                           \\
% \bottomrule
% \end{tabular}
% \caption{Sample Comparison of Human vs T5-DG}
% \end{table}


% \begin{table}[htb!]
% \label{tab:humanscore}
% \begin{tabular}{@{}lllll@{}}
% \toprule
%          & obqa            & tabMCQ        & sciQ            & All             \\ \midrule
% human\_5 & 0.48**          & 0.31          & 0.39*           & 0.48**          \\ \midrule
% KDA\_s   & 0.03            & \textbf{0.14} & \textbf{0.48**} & \textbf{0.43**} \\
% KDA\_h   & 0.08            & 0.1           & 0.38*           & 0.39**          \\ \midrule
% BLEU     & \textbf{0.48**} & 0.01          & 0.13            & 0.21*           \\
% ROUGE-L  & \textbf{0.48**} & 0.09          & 0.08            & 0.24*           \\
% METEOR   & 0.46**          & 0.03          & 0.03            & 0.19            \\ \bottomrule
% \end{tabular}
% \caption{Pearson correlation between metric and human likert score}
% \end{table}


% % from : limitations

% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lcc@{}}
% \toprule
% User response    & Knowledge presence & Knowledge absence \\ \midrule
% Correct answer   & True Positive      & False Positive    \\
% Incorrect answer & False Negative     & True Negative     \\ \bottomrule
% \end{tabular}
% }
% \caption{Confusion matrix for question and knowledge. }
% \label{confusion matrix}
% \end{table}

% \begin{table}[]
% \begin{tabular}{@{}lllll@{}}
% \toprule
%          & obqa  & tabMCQ & sciQ            & All             \\ \midrule
% mol\_tul & -0.16 & 0.04   & \textbf{0.53**} & 0.13            \\
% KD       & 0.04  & 0.16   & \textbf{0.6**}  & \textbf{0.43**}
% \end{tabular}
% \caption{heuristic solver result. correlation to human likert score}
% \end{table}

% % from: appendix

% \begin{table}[]
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|llll}
% \toprule
%   & BLEU1 & BLEU2 & BLEU3 & BLEU4 \\ \midrule
% D1 & 46.59 & 38.33 & 34.31 & 32.02 \\
% D2 & 25.8  & 20.08 & 17.58 & 16.15 \\
% D3 & 28.33 & 23.07 & 20.73 & 19.46 \\ \bottomrule
% \end{tabular}
% \caption{BLEU scores for T5-DG in RACE}
% \label{models}
% \end{table}



% \begin{table}[]
% \small
% \begin{tabular}{@{}llll@{}}
% \toprule
%       & BLEU                                                       & KDA                                                        & Human-likert                                               \\ \midrule
% obqa   & H \textgreater D \textgreater Q \textgreater K & Q \textgreater H = D \textgreater K            & H \textgreater K \textgreater D \textgreater Q \\ 
% tabMCQ & H \textgreater D \textgreater Q \textgreater K & H \textgreater D \textgreater K \textgreater Q & D \textgreater Q \textgreater H \textgreater K \\
% sciQ   & H \textgreater Q \textgreater D \textgreater K & H \textgreater K \textgreater Q \textgreater D & D \textgreater K \textgreater H = Q          \\ \bottomrule
% \end{tabular}
% \normalsize
% \caption{Model Ranking}
% \label{tab: model-ranking}
% \end{table}

==> tables/tab_reproducibility.tex <==
\begin{table*}[t]
\label{badex}
\centering
\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Criteria}}                                                                                                                                                                                                                                  & \textbf{Self-Check}                                           \\ \midrule
\multicolumn{2}{c}{\textbf{For all reported experimental results :}}                                                                                                                                                                                                                                                                   \\ \midrule
A clear description of the mathematical setting, algorithm, and/or model                                                                                                                                                                                               & O (\ref{sec:approach})                                                            \\
\begin{tabular}[c]{@{}l@{}}Submission of a zip file containing source code, with specification of all\\  dependencies, including external libraries, or a link to such resources \\ (while still anonymized) Description of computing infrastructure used\end{tabular} & \begin{tabular}[c]{@{}c@{}}O \\ (Link submitted)\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}The average runtime for each model or algorithm \\ (e.g., training, inference, etc.), or estimated energy cost\end{tabular}                                                                                                                 & Mentioned in \ref{MCQ Solving train}.                                                           \\
Number of parameters in each model                                                                                                                                                                                                                                     & X                                                           \\
Corresponding validation performance for each reported test result                                                                                                                                                                                                     & X                                                           \\
Explanation of evaluation metrics used, with links to code                                                                                                                                                                                                             & O                                                             \\ \midrule
\multicolumn{2}{c}{\textbf{For all experiments with hyperparameter search :}}                                                                                                                                                                                                                                                          \\ \midrule
The exact number of training and evaluation runs                                                                                                                                                                                                                       & 1 (\ref{random forest})                                                           \\
Bounds for each hyperparameter                                                                                                                                                                                                                                         & O (\ref{random forest})                                                           \\
Hyperparameter configurations for best-performing models                                                                                                                                                                                                               & library default (\ref{random forest})                                                           \\
Number of hyperparameter search trials                                                                                                                                                                                                                                 & library default (\ref{random forest})                                                           \\
\begin{tabular}[c]{@{}l@{}}The method of choosing hyperparameter values (e.g., uniform sampling, \\ manual tuning, etc.) and the criterion used to select among them (e.g., accuracy)\end{tabular}                                                                     & O                                                           \\
Summary statistics of the results (e.g., mean, variance, error bars, etc.)                                                                                                                                                                                             & O                                                           \\ \midrule
\multicolumn{2}{c}{\textbf{For all datasets used :}}                                                                                                                                                                                                                                                                                   \\ \midrule
\begin{tabular}[c]{@{}l@{}}Relevant details such as languages, and number of examples and\\  label distributions\end{tabular}                                                                                                                                          & O (\ref{sec:approach})                                                           \\
Details of train/validation/test splits                                                                                                                                                                                                                                & O                                                             \\
Explanation of any data that were excluded, and all pre-processing steps                                                                                                                                                                                               & X                                                           \\
A zip file containing data or link to a downloadable version of the data                                                                                                                                                                                               & O (with code)                                                           \\
\begin{tabular}[c]{@{}l@{}}For new data collected, a complete description of the data collection \\ process, such as instructions to annotators and methods for quality control.\end{tabular}                                                                          & O                                                             \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Reproducibility crieteria self-check table.}
\end{table*}



==> tables/tab_uniformed_solver.tex <==
\begin{table}[]
\begin{tabular}{@{}lllll@{}}
\toprule
                                                                               & OBQA & TabMCQ & SciQ    & All   \\ \midrule
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}uninformed\\ solver\end{tabular}} & 0.16 & -0.04  & -0.53** & -0.13 \\ \bottomrule
\end{tabular}
\caption{Correlation between uninformed solver's correctness probability and the expert likert score. double asterisk
denotes p-value under 0.01}
\end{table}


